Fast full N-body simulations of generic modified gravity: conformal coupling models

We present MG-GLAM, a code developed for the very fast production of full $N$-body cosmological simulations in modified gravity (MG) models. We describe the implementation, numerical tests and first results of a large suite of cosmological simulations for three classes of MG models with conformal coupling terms: the $f(R)$ gravity, symmetron and coupled quintessence models. Derived from the parallel particle-mesh code GLAM, MG-GLAM incorporates an efficient multigrid relaxation technique to solve the characteristic nonlinear partial differential equations of these models. For $f(R)$ gravity, we have included new variants to diversify the model behaviour, and we have tailored the relaxation algorithms to these to maintain high computational efficiency. In a companion paper, we describe versions of this code developed for derivative coupling MG models, including the Vainshtein- and K-mouflage-type models. MG-GLAM can model the prototypes for most MG models of interest, and is broad and versatile. The code is highly optimised, with a tremendous speedup of a factor of more than a hundred compared with earlier $N$-body codes, while still giving accurate predictions of the matter power spectrum and dark matter halo abundance. MG-GLAM is ideal for the generation of large numbers of MG simulations that can be used in the construction of mock galaxy catalogues and the production of accurate emulators for ongoing and future galaxy surveys.

==> Scaling.tex <==
\section{Scalability Test}
\label{sec:scaling}

% We run a series of tests (taking $f(R)$ gravity as a representative) to demonstrate the scaling performace of \textsc{mg-glam} on the SKUN6@IAA facility managed by the IAA-CSIC in Spain.


% The strong scaling tests of \textsc{mg-glam} are presented in the left panel of Fig.~\ref{fig:scaling}. The test simulations employed a fixed resolution of $256^3$ particles and $512^3$ grids, with the same Planck 2015 cosmology as used in the main \textsc{mg-glam} runs of this paper. The plot shows that, when the number of \textsc{openmp} threads ranges between 1 and $\sim 30$, the wallclock time roughly scales linearly with the thread number. The deviation from a linear scaling when the number of threads exceeds $30$ is possibly due to the small size of the test run.

% We also ran a set of simulations of different sizes by varying the resolutions and keeping the number of threads fixed. The wallclock time used is shown in the right panel of Fig.~\ref{fig:scaling}. We see that the time consumption scales nearly perfectly linearly with the considered resolutions (up to $N_{\rm g} = 4096$ and $N_{\rm p} = N_{\rm g} / 2$).


% \begin{figure}
%     \centering 
%     \includegraphics[width=\textwidth]{./fig/scaling.pdf}
%     \caption{
%         \textit{Left panel:} The wallclock time of the \textsc{mg-glam} test runs for the F5n1 model, with fixed simulation size and resolution ($L=128h^{-1}\mathrm{Mpc}$, $N_{\rm p} = 256$, $N_{\rm g} = 512$), as a function of the number of threads used in \textsc{openmp} parallelisation.
%         The time-thread number scaling is approximately linear for thread numbers up to $\sim 30$.
%         \textit{Right panel:} The wallclock time of the \textsc{mg-glam} runs for F5n1 with varying simulation sizes and resolutions (from left to right, $N_{\rm g} = 256, 512, 1024, 2048, 4096$, and $N_{\rm p} = N_{\rm g}/2$), while the number of threads is fixed to \textcolor{red}{$56$}. Again the scaling is linear. In both cases, the symbols denote the times taken by the test runs, and the lines denote the expected results with a `perfect scaling'.
%     }
%     \label{fig:scaling}
% \end{figure}



